On Topology of Three-dimensional Continua with Singular Points

We propose to model the topology of three-dimensional (3D) continua by Yin sets, regular open semianalytic sets with bounded boundary. Our model differs from manifold-based models in that singular points of a 3D continuum, i.e., boundary points where the tangent plane is not uniquely defined, are treated not as anomalies but as a central subject of our theoretical investigation. We characterize the local and global topology of Yin sets. Then we give a unique boundary representation of Yin sets based on the notion of a glued surface, a quotient space of an orientable compact 2-manifold along a one-dimensional CW complex. Our results apply to 3D continua with arbitrarily complex topology and may be useful in a number of scientific and engineering applications such as solid modeling, computer-aided design, and numerical simulations of multiphase flows with topological changes.

==> sec/boolean.tex <==

\subsection{Representing Yin sets
  via realizable spadopags}
\label{sec:repr-yin-sets}

In this subsection,
we propose a space consisting of boundary representations of the Yin sets,
which establishes a one-to-one correspondence with
the Yin space $\mathbb{Y}$.
We start with the following acronym.
\begin{definition}
  A \emph{spadopag} is a nonempty set of
  pairwise almost disjoint, oriented,
  piecewise-analytic glued surfaces.
\end{definition}

We define the boundary-to-interior map $\rho$ as follows, which assigns
a Yin set to each spadopag $\mathcal{G}_{j}$,
\begin{equation}
  \rho(\mathcal{G}_{j}) = \bigcap_{\mathcal{S}_i\in \mathcal{G}}
  \mathrm{int}(\mathcal{S}_{i}).
\end{equation}

According to Theorem \ref{thm:connectedYinsetrep} and Corollary
\ref{coro:Yinsetrep},
not all spadopags are appropriate to represent  Yin sets.
Consequently, we  further propose restrictions on this concept.

\begin{definition}
  \label{def:atom}
  An \emph{atom spadopags} $\mathcal{G}$ is a spadopag 
  that consists of at most one positively oriented glued
  surface $\mathcal{S}^+$ and a finite number of negatively
  oriented glued surfaces
  $\mathcal{S}_1^-, \mathcal{S}_2^-, \cdots, \mathcal{S}_{n_-}^-$
  such that
  \begin{enumerate}[(a)]
  \item $\mathcal{S}_j^-$'s are mutually incomparable with respect
    to inclusion;
  \item $\mathcal{S}_l^- \prec \mathcal{S}^+$, 
    $l = 1, 2, \cdots, n_-$;
    \item $\rho(\mathcal{G})$ is a connected Yin set.
  \end{enumerate}
\end{definition}

Since a spadopag is nonempty, the absence of $\mathcal{S}^+$ means
$n_->0$ and $n_-=0$ implies the presence of $\mathcal{S}^+$.
As a result, an atom spadopag must be one of the two types
$\mathcal{G}^+$ and $\mathcal{G}^-$ in (\ref{equ:setgsurfacetype}).

\begin{definition}
  \label{def:realizable}
  A \emph{realizable spadopag} $\mathcal{G} = \bigcup_k \mathcal{G}_k$ is
  the union of a finite number of atom spadopags, such that for
  any $\mathcal{G}_i$ and $\mathcal{G}_j$,
  $\rho(\mathcal{G}_i) \cap \rho(\mathcal{G}_j) = \emptyset$.
\end{definition}

Based on the boundary-to-interior map $\rho$,
it is natural to observe that an atom spadopag corresponds to
a connected Yin set while a realizable spadopag corresponds to
a general Yin set.

By Corollary \ref{coro:Yinsetrep},
it is straightforward to obtain the
following lemma, which recovers the constitutive atom spadopags
from the realizable spadopag.

\begin{lemma}
  \label{lem:r2a}
  Any realizable spadopag $\mathcal{G}$ can be uniquely expressed as
  \begin{equation}
    \label{equ:bdryrep}
  \mathcal{G} = \mathop{\bigcup}\limits_{i=1}^n
  \mathcal{G}_i^+ \cup \mathcal{G}^-
\end{equation}
where the atom spadopags $\mathcal{G}_i^+$'s and $\mathcal{G}^-$ are
extracted from $\mathcal{G}$
as follows:
\begin{enumerate}[({R2A}-1)]
\item For each positively oriented glued surface
  $\mathcal{S}^+_{j} \in \mathcal{G}$, form an atom spadopag by adding
  $\mathcal{S}^+_{j}$ and all negatively oriented glued surfaces covered
  by $\mathcal{S}_j^+$;
\item If there are negatively oriented glued surfaces left in
  $\mathcal{G}$, group them into an atom spadopag $\mathcal{G}^-$.
\end{enumerate}
\end{lemma}


\begin{figure}
  \centering 
  {\includegraphics[width=0.3\textwidth]{pst/hasse}}
  \caption{The Hasse diagram for the realizable spadopag
    $\mathcal{G} = \left\{ \mathcal{S}_1^+, \mathcal{S}_2^-,
      \mathcal{S}_3^+, \mathcal{S}_4^-, \mathcal{S}_5^- \right\}$ that
    represents the Yin set in Fig \ref{fig:yinsetexm}, where $ \mathcal{S}_1^+$
    and $\mathcal{S}_3^+$ corresponds to the two big blue tori,
    $\mathcal{S}_2^-$, $\mathcal{S}_4^-$ and $\mathcal{S}_5^-$ corresponds to
    the three small white sphere and tori.
    The partial order is the "inclusion" relation as in Definition
    \ref{def:inclusion}.
    A shaded circle represents a positively oriented glued surface while
    an unshaded circle a negatively oriented glued surface.
    The partition of $\mathcal{G}$ into atom spadopags consists of two steps:
    (a) construct an atom spadopag from each shaded circle and its immediate
    children (if there are any) and (b) if any unshaded circle remain,
    group them into $\mathcal{G}^-$.
  }
  \label{fig:hasse}
 \end{figure}

 
\subsection{Classifying Yin sets with their boundaries}
\label{sec:classifying-yin-sets}
 
\begin{definition}
  \label{def:gspace}
  The \emph{G-space} is the set
  \begin{equation}
    \mathbb{G} := \left\{ \hat{0}, \hat{1} \right\} \cup
    \left\{ \mathcal{G} \right\},
  \end{equation}
  where $\left\{ \mathcal{G} \right\}$ denotes the set of
  all realizable spadopags and $\hat{0}, \hat{1}$ are two
  symbols satisfying
  \begin{equation}
    \label{equ:rho01}
    \rho(\hat{0}) = \emptyset, \quad \rho(\hat{1}) = \mathbb{R}^{3}.
  \end{equation}
\end{definition}

Actually $\hat{0}$ and $\hat{1}$ can be interpreted as atom
spadopags which consist of only one oriented glued surface
with  infinitesimal diameter such that
its interior goes to  $\emptyset$ and $\mathbb{R}^3$, respectively.

Now we can extend the definition of the boundary-to-interior map $\rho$
to the G-space.

\begin{definition}
  \label{def:b2imap}
  The boundary-to-interior map $\rho : \mathbb{G} \rightarrow \mathbb{Y}$
  is defined as follows
\begin{equation}
  \rho(\mathcal{G}) :=
   \left\{
    \begin{array}{ll}  
     \emptyset
    \quad &if \,\,\mathcal{G}= \hat{0}; \\
    \mathbb{R}^{3}
      \quad &if \,\,\mathcal{G}= \hat{1};  \\
      \bigcup_{\mathcal{G}_{j}\subset \mathcal{G}}^{\perp\perp}
      \bigcap_{\mathcal{S}_{i}\in \mathcal{G}_j} \mathrm{int}(\mathcal{S}_{i})
      \quad&otherwise,
    \end{array}
    \right.
  \end{equation}
  where the $\mathcal{G}_{j}$'s are the atom spadopags recovered from
  $\mathcal{G}$ as in Lemma \ref{lem:r2a}.
\end{definition}

\begin{lemma}
  \label{lem:rhobijective}
  The boundary-to-interior map $\rho$ in Definition \ref{def:b2imap}
  is bijective.
\end{lemma}
\begin{proof}
For the Yin sets $\emptyset$ and $\mathbb{R}^{3}$,
(\ref{equ:rho01}) shows that $\hat{0}$ and $\hat{1}$ are
their preimages, respectively.
For any other Yin set $\mathcal{Y} \neq \emptyset, \mathbb{R}^{3}$,
by Corollary \ref{coro:Yinsetrep} and Definition \ref{def:realizable},
there exists a preimage in $\mathbb{G}$.
Thus $\rho$ is surjective.
Besides, by Corollary \ref{coro:Yinsetrep} and
Lemma \ref{lem:r2a},
$\rho$ is injective.
%In conclusion, $\rho$ is bijective,  
\end{proof}

Lemma \ref{lem:rhobijective} states that $\rho$ establishes a
one-to-one correspondence between $\mathbb{Y}$ and $\mathbb{G}$.
The realizable spadopag in $\mathbb{G}$ is the unique boundary
representation of the corresponding Yin set in $\mathbb{Y}$.

% \begin{theorem}
%   \label{thm:YinSpaceIsomorphism}
%   The Yin space and the G-space are isomorphic. 
% \end{theorem}

\subsection{Theory} 
We propose the theoretic Boolean algebra on 3D Yin sets in
this subsection.
At the beginning, we introduce three elementary maps, which serve
as the basis of the Boolean operations.
Then we propose the complementation operation and the meet 
operation.
The join operation can be constructed as the composition of
them by the DeMorgan's law.
Finally we prove that the Boolean algebra on $\mathbb{G}$
is isomorphic to that  on $\mathbb{Y}$ with
respect to the boundary-to-interior map $\rho$.

\subsubsection{Three elementary maps}
We define the three maps as follows.

\begin{definition}
  \label{def:cuttingmap}
  Given a realizable spadpog $\mathcal{G}$, the \emph{cutting map}
  $C_{\mathcal{I}}$
  produces the corresponding segmented realizable spadpog
  $C_{\mathcal{I}}(\mathcal{G})$ as follows:
  \begin{enumerate}[({R2S}-1)]
  \item Apply the intersection detection method to obtain
    all intersections of the glued surfaces in $\mathcal{G}$, denoted as
    $\mathcal{I}$.
  \item For each  glued surface $\mathcal{S}$ in $\mathcal{G}$,
    segment $\mathcal{S}$ at its intersections in $\mathcal{I}$
    and add the segmented parts to $C_{\mathcal{I}}(\mathcal{G})$;
  \end{enumerate}
\end{definition}


Notice that a segmented realizable spadpog may include
segmented surface patches and closed glued surfaces.
The  normal vector of any point on the surface patch coincides
with that of the same point on the original glued surface.
In addition, for a boundary curve of a surface patch,
its orientation is decided by the  normal vector
of any point in a small neighborhood of the curve together with
the right-hand rule.

\begin{definition}
  \label{def:pastingmap}
  Given a segmented realizable spadpog $C_{\mathcal{I}}(\mathcal{G})$,
  the \emph{pasting map} $C^{-1}_{\mathcal{I}}$
  constructs the corresponding  realizable spadpog
  $\mathcal{G}$ as follows:
  \begin{enumerate}[({S2R}-1)]
  \item Remove all glued surfaces in $C_{\mathcal{I}}(\mathcal{G})$
    and insert them into $\mathcal{G}$.
  \item Start with a surface patch $\beta$ in  $C_{\mathcal{I}}(\mathcal{G})$.
    For a boundary curve $\gamma$ of $\beta$, find all surface patches that
    share $\gamma$ but have the opposite orientation, denoted
    as $\mathcal{N}_{\beta}(\gamma)$.
    Choose a point $p$ on $\gamma$ and calculate the normal
    vector of $p$ with respect to $\beta$, denoted as $n_A$.
    For $\beta'$ in $\mathcal{N}_{\beta}(\gamma)$, calculate
    the normal vector of $p$, denoted as $n_{B}$.
    The angle between $n_A$ and $n_B$ is $\alpha$.
    Let $r_p$ be the direction vector of $\gamma$ at $p$.
    If $(n_A\times n_{B})\cdot r_p > 0 $, the directed angle $\theta$
    between $\beta$ and $\beta'$ is $\pi- \alpha$,
    otherwise  $\theta = \pi + \alpha$.
    Choose the surface patch in $\mathcal{N}_{\beta}(\gamma)$ such that
    $\theta$ attains the minumum and glue it to $\beta$.
    Repeat the above steps until $\beta$ is glued into a closed surface
    $\mathcal{C}$
    and remove the glued surface patches in $C_{\mathcal{I}}(\mathcal{G})$.
  \item If $\mathcal{C}$ has no self-intersections, add it into
    $\mathcal{G}$; otherwise divide $\mathcal{C}$ into glued surfaces
    by the dividing map in Definition \ref{def:dividingmap}
    and insert them into $\mathcal{G}$.
    \item Repeat (S2R-2,3) until $C_{\mathcal{I}}(\mathcal{G})$ is empty.
  \end{enumerate}
\end{definition}

\begin{figure}[H]
  \centering 
  \subfigure[A big ellipsoid with a small ellipsoid removed
  from it such that the larger one is tangent to the smaller one
  at a circle]{\includegraphics[width=0.3\textwidth]{png/pastingmap1}}
  \hspace{20mm}
  \subfigure[The segmented realizable spadpog from (a), which consists
  of four surface patches]
  {\includegraphics[width=0.3\textwidth]{pst/pastingmap}}
  \caption{Illustrating the pasting map in Definition \ref{def:pastingmap}.
    Starting from
    $\beta$, we pick $\beta'$ to glue at the boundary curve (which
    is represented by a solid dot), in that $\theta$ attains the minimum.
    Finally, all surface patches are pasted into two glued surfaces
    with an improper intersection as a circle, which is consistent with
    the boundary representation in Corollary \ref{coro:Yinsetrep}
    since the Yin set in (a) has exactly two components.
  }
  \label{fig:pastingmap}
 \end{figure}

\begin{definition}
  \label{def:dividingmap}
  For a closed surface $\mathcal{C}$ obtained from (S2R-2), we design the
  dividing map to divide $\mathcal{C}$ into a set of glued surfaces
  $\mathcal{G}$ as follows:
  \begin{enumerate}[({C2G}-1)]
  \item Segment $\mathcal{C}$ at its self-intersections $\mathcal{I}$ and 
    the segmented surface patches form a set
    $C_{\mathcal{I}}(\left\{ \mathcal{C} \right\})$.
  \item Reverse the orientation of each surface patch in
    $C_{\mathcal{I}}(\left\{ \mathcal{C} \right\})$ by reversing the
    direction of the normal vector at each point of the surface patch.
  \item Start with a surface patch in
    $C_{\mathcal{I}}(\left\{ \mathcal{C} \right\})$,
    follow (S2R-2) to glue it into a closed surface
    (which is definitely a glued surface), reverse its orientation
    and then insert it into $\mathcal{G}$.
  \item Repeat (C2G-3) until all surface patches in
    $C_{\mathcal{I}}(\left\{ \mathcal{C} \right\})$ are glued.
  \end{enumerate}
\end{definition}



 
\begin{theorem}
  \label{thm:pastingmap}
  Suppose $C_{\mathcal{I}}(\mathcal{G})$ is a segmented realizable spadpog
  segmented from the realizable spadpog $\mathcal{G}$.
  Then the pasting map in Definition \ref{def:pastingmap} paste
  $C_{\mathcal{I}}(\mathcal{G})$ back to $\mathcal{G}$.
\end{theorem}

\textit{Proof}. The pasting methods in \textit{(S2R-2)} and
\textit{(C2G-3)} are the same as those
in the proof of Theorem \ref{thm:connectedYinsetrep}
in that surface patches glue along the interior of the Yin set in
\textit{(S2R-2)}
while surface patches glue along the exterior of the Yin set
in \textit{(C2G-3)}.
Then by the arguments in  Theorem \ref{thm:connectedYinsetrep},
the pasting map together with the dividing map glues the surface patches
into a series of glued surfaces,
which are mutually almost disjoint.
In the meantime, orientation of these glued surfaces are unchanged such that
the outward normal vector at any point of them always points at
the exterior of the Yin set,
since \textit{ (C2G-2)} and \textit{(C2G-3)} reverse the orientation twice.
Consequently, these glued surfaces constitute a
series of atom spadpogs
by Theorem \ref{thm:connectedYinsetrep} and Definition
\ref{def:atom},  
and form a realizable spadpog by Definition \ref{def:realizable}.
The realizable spadpog must be $\mathcal{G}$ by the uniqueness.

Theorem \ref{thm:pastingmap} shows that the pasting map is the
inverse of the cutting map, thus our usage of $"C^{-1}_{\mathcal{I}}"$
makes sense.


\subsubsection{Complementation: A unitary operation on $\mathbb{G}$}
The complementation operation is constructed from the composition of
the cutting map, the orientation reversing map and the pasting map.

\begin{definition}
  \label{def:complement}
  The complementation operation $' : \mathbb{G} \rightarrow \mathbb{G}$
  is defined as
  \begin{equation}
    \label{equ:complement}
    \mathcal{G}' :=
   \left\{
    \begin{array}{ll}  
     \hat{1}
    \quad &if \,\,\mathcal{G}= \hat{0}; \\
    \hat{0}
      \quad &if\,\, \mathcal{G}= \hat{1};  \\
     \left( C^{-1}_{\mathcal{I}} \circ R \circ C_{\mathcal{I}} \right) \mathcal{G}
      \quad&otherwise,
    \end{array}
    \right.
  \end{equation}
  where $\mathcal{I}$ is the set of improper intersections of glued
  surfaces in $\mathcal{G}$, and the orientation-reversing map $R$
  reverses the orientation of each surface patch as well as 
  each glued surface in $C_{\mathcal{I}}(\mathcal{G})$.
\end{definition}

\begin{lemma}
  \label{lem:complement}
  The complementation operation in Definition \ref{def:complement}
  satisfies
  \begin{equation}
    \forall \mathcal{G} \in \mathbb{G}, \quad
    \rho(\mathcal{G}') = (\rho(\mathcal{G}))^{\perp}.
\end{equation}
\end{lemma}

\textit{Proof}. By Theorem \ref{thm:pastingmap}, $\mathcal{G}'$
in (\ref{equ:complement}) is indeed a realizable spadpog,
hence $\rho$ can perform on $\mathcal{G}'$.
By the definition of $\rho$, we only need to prove that
$\mathcal{G}'$ and $\mathcal{G}$ constitute the same boundary
while the corresponding normal vectors on their glued surfaces
have opposite directions.
This is clear since $'$ operation in (\ref{equ:complement})
never inserts or deletes the boundary and orientations of
the surface patches are reversed exactly once by $R$.

Notice that directly reversing the orientation of each glued surface
cannot assure the image is still a realizable spadpog.
See Fig \ref{fig:pastingmap} for example, directly reversing
orientations of the two positively oriented glued surfaces
produces two negatively oriented glued surface, which does not
form a realizable spadpog since the complement of the Yin set
has two connected components, one bounded and one unbounded.

\subsubsection{Meet: A binary operation on $\mathbb{G}$}

To implement the meet of two realizable spadpogs
$\mathcal{G}_1$ and $\mathcal{G}_{2}$,
we cut them by $C_{\mathcal{I}}$, select those surface patches
that belong to the boundary of the Yin set
$\rho(\mathcal{G}_1) \cap \rho(\mathcal{G}_2)$,
and use $C_{\mathcal{I}}^{-1}$ to paste these surface patches into
a realizable spadpog.
Lemma \ref{lem:meetchoose} and Corollary \ref{coro:meetchoose}
tell us which surface patches we should choose.

\begin{lemma}
  \label{lem:meetchoose}
  Denote $\mathcal{Y} := \mathrm{int}(\mathcal{S}_1) \cap
  \mathrm{int}(\mathcal{S}_{2})$,
  where $\mathcal{S}_1$ and $\mathcal{S}_2$ are two
  oriented glued surfaces.
  For a surface patch $\beta$ satisfying
  $\beta \subset \mathcal{S}_1$ and $\beta \subset
  \mathbb{R}^3\backslash \mathcal{S}_2$,
  we have $\beta \subset \partial \mathcal{Y}$ if and only if
  $\beta \subset \mathrm{int}(\mathcal{S}_2)$.
  For a surface patch $\beta$ satisfying
  $\beta \subset \mathcal{S}_1\cap \mathcal{S}_2$,
  we have $\beta \subset \partial \mathcal{Y}$ if and only if
   orientation of $\beta$ induced from  orientation of $\mathcal{S}_{1}$
  is the same as that induced from  orientation of $\mathcal{S}_{2}$.
\end{lemma}

\textit{Proof}. We only prove the first statement since the second one can be
similarly shown.
For the sufficiency, to prove $\beta \subset \partial\mathcal{Y}$,
we only need to prove that $\forall p \in \beta$, for any neighborhood
$\mathcal{N}(p)$ of $p$, $\mathcal{N}(p) \cap \mathcal{Y} \neq \emptyset$
and $\mathcal{N}(p) \cap \mathcal{Y}^{\perp} \neq \emptyset$.
From $\beta \subset \mathcal{S}_1$ and $\beta \subset
\mathrm{int}(\mathcal{S}_2)$,
we have $\mathcal{N}(p) \cap \mathrm{int}(\mathcal{S}_1) \neq \emptyset$
and $\mathcal{N}(p) \cap \mathrm{int}(\mathcal{S}_2) \neq \emptyset$,
respectively, which further yields
$\mathcal{N}(p)\cap \mathcal{Y}
\neq \emptyset$.
Since $\beta \subset \mathcal{S}_1$,
$\mathcal{N}(p) \cap
\mathrm{int}(\mathcal{S}_1)^{\perp} \neq \emptyset$,
then we have $\mathcal{N}(p)\cap \mathcal{Y}^{\perp}\neq \emptyset$.
Thus $\beta \subset \partial \mathcal{Y}$.
For the necessity, suppose $\beta \not\subset \mathrm{int}(\mathcal{S}_{2})$.
Since $\beta \subset \mathbb{R}^{3}\backslash \mathcal{S}_2$,
$\beta \subset \mathrm{ext}(\mathcal{S}_2)$.
Then we have $\beta \subset \mathcal{Y}^{\perp}$, which contradicts the fact
that $\beta \subset \partial\mathcal{Y}$.
This completes the proof.



Hereafter we denote the union of all glued surfaces in a realizable
spadpog $\mathcal{G}$ as
\begin{equation}
  \label{equ:unionrealizable}
  P(\mathcal{G}) := \mathop{\bigcup}\limits_{\mathcal{S}_i\in \mathcal{G}}
  \mathcal{S}_{i},
\end{equation}
which is a subset of $\mathbb{R}^{3}$.
Similar arguments lead to the following corollary.
\begin{corollary}
  \label{coro:meetchoose}
  Denote $\mathcal{Y}:= \rho(\mathcal{G}_1) \cap \rho(\mathcal{G}_2)$,
  where $\mathcal{G}_1$ and $\mathcal{G}_2$ are two realizable spadpogs.
  For a surface patch $\beta$ satisfying $\beta \subset P(\mathcal{G}_{1})$
  and $\beta \subset \mathbb{R}^3\backslash P(\mathcal{G}_{2})$,
  we have $\beta \subset \partial \mathcal{Y}$ if and only if
  $\beta \subset \rho(\mathcal{G}_{2})$.
  For a surface patch $\beta$ satisfying $\beta \subset
  P(\mathcal{G}_1)\cap P(\mathcal{G}_2)$,
  we have $\beta \subset \partial \mathcal{Y}$ if and only if
  orientation of $\beta$ induced from  orientation of $\mathcal{G}_{1}$
  is the same as that induced from orientation of $\mathcal{G}_{2}$.
\end{corollary}


\begin{definition}
  \label{def:meet}
  The meet of two realizable spadpogs $\mathcal{G}_1$ and $\mathcal{G}_2$
  is a binary operation $\wedge: \mathbb{G} \times \mathbb{G} \rightarrow
  \mathbb{G}$ defined  as
  \begin{equation}
    \mathcal{G}_1 \wedge \mathcal{G}_2 =
     \left\{
    \begin{array}{ll}  
     \hat{0}
    \quad &if\,\, \mathcal{G}_{2}= \hat{0}; \\
    \mathcal{G}_{1}
      \quad &if\,\, \mathcal{G}_{2}= \hat{1};  \\
     C^{-1}_{\mathcal{I}}(E) 
      \quad&otherwise,
    \end{array}
    \right.
  \end{equation}
  where the intersection set $\mathcal{I}$ and the segmented realizable
  spadpog $E$ are constructed as follows:
  \begin{enumerate}[({MRS}-1)]
  \item Apply the intersection detection method to obtain intersections
    between and within
    $\mathcal{G}_1$ and $\mathcal{G}_2$, denoted as $\mathcal{I}$.
  \item Apply the cutting map to $\mathcal{G}_1$ and $\mathcal{G}_2$
    with intersections $\mathcal{I}$, resulting segmented realizable
    spadpogs $C_{\mathcal{I}}(\mathcal{G}_1)$ and $C_{\mathcal{I}}(\mathcal{G}_{2})$,
    respectively.
  \item For each $\beta \in C_{\mathcal{I}}(\mathcal{G}_1)$,
    insert it into $E$ if $\beta$ minus its boundary is contained in
    $\rho(\mathcal{G}_{2})$, or if there exists
    $\beta'\in C_{\mathcal{I}}(\mathcal{G}_2)$ such that
    $\beta =\beta'$ and they have the same orientation.
    \item For  each $\beta \in C_{\mathcal{I}}(\mathcal{G}_2)$,
    insert it into $E$ if $\beta$ minus its boundary is contained in
    $\rho(\mathcal{G}_{1})$.
  \end{enumerate}
\end{definition}

\begin{lemma}
  \label{lem:meet}
  The meet operation in Definition \ref{def:meet} satisfies
  \begin{equation}
    \label{equ:meet}
    \forall \mathcal{G}_1, \mathcal{G}_2 \in \mathbb{G},\quad
    \rho(\mathcal{G}_1\wedge \mathcal{G}_2) =
    \rho(\mathcal{G}_1) \cap \rho(\mathcal{G}_{2}).
\end{equation}
\end{lemma}

\textit{Proof}. From Theorem \ref{thm:pastingmap},
$\mathcal{G}_1\wedge \mathcal{G}_2$ in (\ref{equ:meet})
is indeed a realizable spadpog, which can be acted upon
by $\rho$.
By Corollary \ref{coro:meetchoose}, the union of the
surface patches chosen in (MRS-3,4) equals to
$\partial(\rho(\mathcal{G}_1) \cap \rho(\mathcal{G}_{2}))$.
Also, the outward normal vector of any point always points at the
exterior of $ \rho(\mathcal{G}_1) \cap \rho(\mathcal{G}_{2})$
since orientation of any surface patch is not changed in the
meet process.
The proof is then completed by the definition of $\rho$.

\subsubsection{Isomorphism}

The join operation can be implemented by composing the meet operation
and the complementation operation;
this also works for all other Boolean operations.

\begin{definition}
  \label{def:join}
  The join of two realizable spadpogs $\mathcal{G}_1$ and $\mathcal{G}_{2}$
  is a binary operation $\vee: \mathbb{G}\times \mathbb{G} \rightarrow
  \mathbb{G}$ defined as
  \begin{equation}
    \forall \mathcal{G}_1, \mathcal{G}_2 \in \mathbb{G},\quad
    \mathcal{G}_1\vee \mathcal{G}_2 :=
    \left( \mathcal{G}_1' \wedge \mathcal{G}_2' \right)'.
\end{equation}
\end{definition}

Based on  Definition \ref{def:join},
Lemma \ref{lem:complement}, Lemma \ref{lem:meet}
and DeMorgan's law, it is
straightforward to obtain the following lemma.
\begin{lemma}
  \label{lem:join}
  The join operation in Definition \ref{def:join} satisfies
  \begin{equation}
    \forall  \mathcal{G}_1, \mathcal{G}_2 \in \mathbb{G},\quad
    \rho(\mathcal{G}_1 \vee \mathcal{G}_2) =
    \rho(\mathcal{G}_1) \cup \rho(\mathcal{G}_{2}).
\end{equation}
\end{lemma}

The following theorem is the theoretical culmination of this paper.

\begin{theorem}
  \label{thm:isomorphism}
  The Boolean algebras $\left( \mathbb{Y}, \cup^{\perp\perp}, \cap,
   ^{\perp}, \emptyset, \mathbb{R}^3\right)$ and
  $\left(\mathbb{G}, \vee, \wedge, ', \hat{0}, \hat{1}  \right)$
  are isomorphic under the boundary-to-interior map $\rho$ in
  Definition \ref{def:b2imap}.
\end{theorem}

\textit{Proof}: This follows directly from Theorem \ref{thm:rhobijective},
Lemma \ref{lem:complement}, Lemma \ref{lem:meet} and Lemma \ref{lem:join}.

From Theorem \ref{thm:isomorphism}, we do not have to perform Boolean
operations directly on the Yin sets, which costs a substantial amount
of time and memory.
Instead, we perform efficient Boolean operations
on the realizable spadpogs and
then use $\rho$ to recover the corresponding Yin sets.

\subsection{Design}
In this subsection, we discuss the details on the algorithmic design
and implementations of the Boolean algebra.
We do not expect the reader to implement all algorithms after reading
this subsection.
Instead, we intend to paint a relatively complete picture on the
designing of the Boolean algorithms for the reader.

\subsubsection{User-friendly design}
In the implementation, each Yin set is represented by a
realizable spadpog and each glued surface in a realizable spadpog
is approximated by a closed triangulation.
To construct a Yin set, an .obj file is usually inputted, which contains
information of  triangles of each glued surface.
The user is not required to specify the inclusion relations of these
glued surfaces in that  computation of this information has
been encapsulated within the algorithms.
As long as each input is indeed a realizable spadpog,
our algorithm provides the correct result.
Additionally, the user has the option to output the results
in the same format as the input or generate the Hasse diagram
of the results based on the inclusion relations.
These designs ensure that the software interface is simple, flexible
and user-friendly.



\subsubsection{Robustness}
Our algorithms adhere to an important criterion throughout the design process:
\textit{Given a small positive real number $\epsilon$, we define
  two points to be the same point if their distance is smaller than
  $\epsilon$.}

\begin{figure}[H]
  \centering
  \subfigure[$\mathcal{Y}_{1}$: represented by a positively oriented torus]
  {\includegraphics[width=0.4\textwidth]{png/complextopology2}}
  \hspace{10mm}
  \subfigure[$\mathcal{Y}_{2}$: represented by two negatively
  oriented glued surfaces, where the ball and
  the torus are connected by a thin pipe to form a glued surface
  ]
  {\includegraphics[width=0.4\textwidth]{png/complextopology1}}

  \subfigure[$\mathcal{Y}_1 \cap \mathcal{Y}_2$:
  represented by two positively oriented glued surfaces]
  {\includegraphics[width=0.6\textwidth]{png/complextopologymeet}}
  \caption{Results of testing Boolean operations on Yin sets
    with complex topology.
    All of the two balls and one torus in (b) are tangent to the big torus
    in (a) at a circle.
    Then the meet operation produce two positively oriented glued surfaces
    in (c), which are colored red and blue, respectively.
}
 \label{fig:complextopology}
\end{figure}


Enforcing this criterion not only eliminites the impact of round-off errors,
but also handles the extreme cases in computational geometry,
like calculating intersections of line segments in an unlimited
range of length scales.
Besides, this criterion can  be extended to
deal with intersecting two triangles or
determining whether two vectors are parallel.
The key point is to make the whole algorithm as robust
and consistent as possible.


\subsubsection{Implementation}
To implement the cutting map $C_{\mathcal{I}}$ in Definition
\ref{def:cuttingmap},
an indispensable part is intersecting two glued surfaces,
which are represented by closed triangulations.
We compute the intersection lines for each pair of potentially
intersecting triangles and retriangulate each triangle with
respect to its intersection lines, such that every surface patch
obtained from the cutting map still forms a triangulation.

Pairwise calculating the intersections of triangles in the two glued surfaces
 involves a significant amount of computation.
In the two-dimensional case,
the sweep line algorithm is applied to 
get the intersections of a set of segments,
where unnecessary tests for segment-segment pairs
that are far away from each other are prevented.
The same idea applies in the three-dimensional case.
We apply an adaptive octree-based method \cite{wong14:_collision_detection}.
The region containing all triangles is continually subdivided into
cells, which is organized by a octree.
From top to bottom, each triangle is assigned to the cells it intersects.
To further reduce the number of intersection tests,
cells are adaptively merged from bottom to top.
Finally, a intersection test is performed on two triangles if and only if
they are in the same cell, that is, they are adjacent.

As for implementing the pasting map $C_{\mathcal{I}}^{-1}$,
a basic problem is determining the relative position of a set of
points to a glued surface.
We use the ray-crossing algorithm in \cite{rourke98:_computational_geometry}.
To be more specific, for a query point $q$, a ray from $q$ to
infinity is randomly generated. $q$ is inside the glued surface
if and only if the ray crosses the glued surface an odd number of
times.
Notice that degeneracies may emergy when a ray crosses a glued surface,
such as the ray may collinearly overlap with an edge,
which is troublesome.
We handle these degeneracies by keeping
generating random rays until no degeneracies happen.



\subsection{Applications}
In this subsection, we display the applications of the Yin sets and the
Boolean algebra.

\begin{figure}[H]
  \centering
  \subfigure[$\mathcal{Y}_{1}$: an armadillo
  represented by a positively oriented glued surface]
  {\includegraphics[width=0.4\textwidth]{png/complexgeometry1}}
  \hspace{10mm}
  \subfigure[$\mathcal{Y}_{2}$: an rabbit represented by
  a positively oriented glued surface
  ]
  {\includegraphics[width=0.4\textwidth]{png/complexgeometry2}}

  \subfigure[$\mathcal{Y}_1 \cap \mathcal{Y}_2$:
  represented by a positively oriented glued surface]
  {\includegraphics[width=0.4\textwidth]{png/complexgeometrymeet}}
  \hspace{10mm}
   \subfigure[$\mathcal{Y}_1 \cup \mathcal{Y}_2$:
  represented by a positively oriented glued surface]
  {\includegraphics[width=0.4\textwidth]{png/complexgeometryjoin}}
  \caption{Results of testing Boolean operations on Yin sets
    with complex geometry.
}
 \label{fig:complexgeometry}
\end{figure}


\subsubsection{Applications to modeling}
Boolean operations are indispensable in 3D modeling
in that a lot of complex models can be
constructed by applying a series of Boolean operations
to some very simple models.
Based on the theory in this section, our Boolean operations are
applicable to any Yin set, no matter how complex their geometry or
topology is.
We display two typical tests as follows.
In Fig \ref{fig:complextopology}, the meet of the two Yin sets involves
multiple improper intersections which affect the number of
connected components in the result.
Our algorithm produces two positively oriented glued surface, which
coincides with the boundary representation in (\ref{equ:bdryrep})
since the result has exactly two components without any holes.
Fig \ref{fig:complexgeometry} shows the results of Boolean operations
on an armadillo (which can be downloaded from
the Stanford 3D scanning reposity) and a rabbit.
Both of them have complex geometry and our algorithms  produce the
correct results.





\subsubsection{Applications to interface tracking}
\begin{figure}[H]
  \centering
  \subfigure[$t=0$]{\includegraphics[width=0.4\textwidth]{png/IT1}}
  \subfigure[$t=\frac{1}{8}T$]
  {\includegraphics[width=0.4\textwidth]{png/IT2}}

  \subfigure[$t=\frac{1}{4}T$]
  {\includegraphics[width=0.4\textwidth]{png/IT3}}
  \subfigure[$t=\frac{1}{2}T$]
  {\includegraphics[width=0.4\textwidth]{png/IT4}}

  \subfigure[$t=\frac{3}{4}T$]
  {\includegraphics[width=0.4\textwidth]{png/IT5}}
  \subfigure[$t=T$]
  {\includegraphics[width=0.4\textwidth]{png/IT6}}
  \caption{Results of the linear $\mathrm{MARS}$ method for the deformation
    test \cite{leveque96:_high-reso_cons_algo}
    with $T= 3$, $h_L=\frac{1}{128}$, $r_{\mathrm{tiny}}=0.1$, and
  the Happy Buddha (which can be downloaded from the Stanford
  3D scanning repository) in (a) as  the initial condition.
  Over all time steps, the topological structure remains unchanged.
  Besides, geometric features are well recovered in (f).
}
 \label{fig:ITbuddha}
\end{figure}

In an interface tracking (IT) problem, a deforming fluid phase
$\mathcal{M}(t)$ is usually represented by a point set:
$$\mathcal{M}(t) := \left\{ \mathbf{x}: f(\mathbf{x},t)=1 \right\},$$
where $f$ is the color function.
We have to determine
$\mathcal{M}(T)$ based on the initial fluid phase $\mathcal{M}(t_0)$
and the given velocity field $\mathbf{u}(\mathbf{x},t), \,\,t\in
\left[t_0, T  \right]$.
In fact, Yin sets serve as an appropriate mathematical model to
describe the fluid phases.
On the one hand, Yin sets support dealing with topological issues.
On the other hand, Yin sets are equipped with solid theoretical
foundation for analysis in the IT problem.
Based on the Yin sets, we define the IT problem as follows. 
\begin{definition}
  \label{def:IT}
  The \emph{IT} problem is the determination of a Yin set
  $\mathcal{M}(T)\in \mathbb{Y}$ from its initial condition
  $\mathcal{M}(t_0) \in \mathbb{Y}$ under passive advection
  of a nonautonomous ODE,
  \begin{equation}
\frac{d \mathbf{x}}{dt} = \mathbf{u}(\mathbf{x},t),
\end{equation}
where $t$ is the time, $\mathbf{x}(t)\in \mathcal{M}(t)$ is the position
of a passively advected Lagrangian particle in the Yin set,
and $\mathbf{u}$ is continuous in $t$ and Lipschitz continuous in
$\mathbf{x}$.
\end{definition}

We have designed the linear MARS method for 3D IT problems in
Definition \ref{def:IT}.
Given $\mathcal{M}^n \approx \mathcal{M}(t_n)$, major steps
of our IT methods are as follows:
\begin{enumerate}[({IT}-1)]
\item Apply the flow map to vertices of triangulations that
  represent $\mathcal{M}^n \in \mathbb{Y}$ and retain the topological
  connectivity to obtain the Yin set $\mathcal{M}^{n+1}$.
\item Split or collapse edges in $\mathcal{M}^{n+1}$
  if lengths of them are too
  long or too short, respectively, so that lengths of all edges in
  $\mathcal{M}^{n+1}$ are within the interval
  $\left[ r_{\mathrm{tiny}}h_L, h_L \right]$.
\item Adjust the vertex positions and the topological connectivity
  of the triangulations in $\mathcal{M}^{n+1}$
  such that interior angles of all
  triangles in $\mathcal{M}^{n+1}$ are greater than $\alpha$.
\item Apply the meet operation to $\mathcal{M}^{n+1}$ and  fixed
  control volumes of length $h$ to obtain local solutions if needed.
\end{enumerate}

We emphasize that the local solutions play a vital role in
coupling IT with  numerical solvers when dealing with
irregular boundary problems and even moving boundary problems.

In Fig \ref{fig:ITbuddha}, we show results of the deformation test to
demonstrate that the complex geometric features as well as the
topological structure are well preserved  under the homeomorphic
flow map.
We report the details of this coupled method in another paper.


%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:


==> sec/preliminaries.tex <==
\subsection{Regular semianalytic sets}
\label{sec:regularSets}

In a topological space ${\mathcal X}$,
 the \emph{complement} of a subset ${\mathcal P}\subseteq {\mathcal X}$,
 written ${\mathcal P}'$,
 is the set ${\mathcal X}\setminus {\mathcal P}$.
% A subset of ${\mathcal X}$
%  is \emph{closed} if its complement is open.
The \emph{closure} of a set ${\mathcal P}\subseteq{\mathcal X}$,
 written $\overline{{\mathcal P}}$,
 is the intersection of all closed 
 supersets of ${\mathcal P}$.
The \emph{interior} of ${\mathcal P}$, written ${\mathcal P}^{\circ}$,
 is the union of all open subsets of ${\mathcal P}$.
% in ${\mathfrak T}$.
The \emph{exterior} of ${\mathcal P}$,
 written ${\mathcal P}^{\perp}:= {\mathcal P}^{\prime\circ}
 :=({\mathcal P}')^{\circ}$,
 is the interior of its complement.
By the identity $\overline{{\mathcal P}} ={\mathcal P}^{\prime\circ\prime}$
 \cite[p. 58]{givant09:_introd_boolean_algeb},
 we have 
 ${\mathcal P}^{\perp}={\overline{\mathcal P}}^{\prime}$.
A point $\mathbf{x}\in {\mathcal X}$ is
 a \emph{boundary point} of ${\mathcal P}$
 if $\mathbf{x}\not\in {\mathcal P}^{\circ}$
 and $\mathbf{x}\not\in {\mathcal P}^{\perp}$.
The \emph{boundary} of ${\mathcal P}$, written $\partial {\mathcal P}$,
 is the set of all boundary points of ${\mathcal P}$.
It can be shown that
 ${\mathcal P}^{\circ}={\mathcal P}\setminus \partial {\mathcal P}$
 and
 ${\overline{\mathcal P}}= {\mathcal P}\cup \partial {\mathcal P}$.
%
An open set ${\mathcal P}\subseteq {\mathcal X}$ is \emph{regular} if
 it coincides with the interior of its own closure,
 i.e. if ${\mathcal P}={\overline{\mathcal P}}^{\circ}$.
A closed set ${\mathcal P}\subseteq {\mathcal X}$ is \emph{regular} if
 it coincides with the closure of its own interior,
 i.e. if ${\mathcal P}=\overline{{\mathcal P}^{\circ}}$.
The duality of the interior and closure operators
 implies
 ${\mathcal P}^{\circ} =\overline{{\mathcal P}^{\prime}}^{\prime}$,
 hence ${\mathcal P}$ is a \emph{regular open set}
 if and only if ${\mathcal P}={\mathcal P}^{\perp\perp}
 :=\left({\mathcal P}^{\perp}\right)^{\perp}$.
For any subset $Q\subseteq{\mathcal X}$,
 it can be shown that $Q^{\perp\perp}$ is a regular open set
 and $\overline{Q^{\circ}}$ is a regular closed set.

Regular sets, open or closed, capture the salient feature 
 that physically meaningful regions
 are free of lower-dimensional elements
 such as isolated points and curves in 2D
 and dangling faces in 3D.

%  \begin{theorem}[MacNeille \cite{macneille37:_partial}
%    and Tarski \cite{tarski37:_ueber_mengen_mengen}]
%    \label{thm:regularOpenAlgebra}
%    Let ${\mathbb B}$ denote
%     the class of all regular open sets
%     of a topological space ${\mathcal X}$
%     and define
%     ${\mathcal P}\cup^{\perp\perp}{\mathcal Q}
%     := ({\mathcal P}\cup {\mathcal Q})^{\perp\perp}$
%     for all ${\mathcal P},{\mathcal Q}\subseteq {\mathcal X}$.
%    Then
%     $\mathbf{B}_o:=({\mathbb B},\ \cup^{\perp\perp},\ \cap,\ \, ^{\perp},\
%     \emptyset,\ {\mathcal X})$
%     is a Boolean algebra.
%  \end{theorem}
%  \begin{proof}
%    See \cite[\S 10]{givant09:_introd_boolean_algeb}.
%  \end{proof}

% Similarly, it can be shown that,
%  with appropriately defined operations,
%  regular closed sets
%  of a topological space ${\mathcal X}$
%  also form a Boolean algebra
%  \cite[p. 39]{kuratowski76:_set_theor_introd_descr_set_theor}.

Regular sets are not perfect for representing
 physically meaningful regions yet: 
 some of them
 cannot be described by a finite number of symbol structures.
For example, some sets
 have nowhere differentiable boundaries,
 which, in their parametric forms,
 are usually infinite series of continuous functions
 \cite{sagan92:_elemen_proof_schoen_space_fillin}.
Another pathological case
 is more subtle:
 intersecting two regular sets with piecewise smooth boundaries
 may yield an infinite number of disjoint regular sets.
Consider 
 \begin{equation}
   \label{eq:pathologicalIntersection}
   \left\{
   \begin{array}{l}
   {\mathcal A}_p := \{(x,y)\in \mathbb{R}^2 :
    -2< y< \sin\frac{1}{x},\ 
    0< x< 1 \},\\
   {\mathcal A}_s := \{(x,y)\in \mathbb{R}^2 :
    0 < y < 1,\ 
    -1< x< 1 \}.
   \end{array}
   \right.
 \end{equation}

Although both ${\mathcal A}_p$ and ${\mathcal A}_s$
 are described by two inequalities,
 their intersection
 is a disjoint union of an infinite number of regular sets;
 see
 \cite[Fig. 4-1, Fig. 4-2]{requicha77:_mathem_model_rigid_solid_objec}.
This poses a fundamental problem
 that results of Boolean operations of two regular sets
 may not be well represented on a computer
 by a finite number of entitites.

Therefore, %The above discussion entails
 we need to find a proper subspace of regular sets,
 each element of which is finitely describable.
This search eventually
% \footnote{
% The exclusion of nonphysical regular closed sets
%  involves the triangulation of a topological space
%  into a simplicial complex
%  and imposing certain conditions on the embedding
%  of the resulting topological polyhedron
%  in three or higher dimensions;
%  see \cite[Sec. 4.2]{requicha77:_mathem_model_rigid_solid_objec}
%  for an accessible exposition.
% }
 arrives at semianalytic sets.

\begin{definition}
  \label{def:semianalytic-sets}
  A set ${\mathcal S}\subseteq\mathbb{R}^{\Dim}$ is \emph{semianalytic}
   if there exist a finite number of 
   analytic functions $g_i:\mathbb{R}^{\Dim}\rightarrow \mathbb{R}$
   such that ${\mathcal S}$ is in the universe
   of a finite Boolean algebra formed from the sets
   \begin{equation}
     \label{eq:semiAnalyticForm}
     {\mathcal X}_i=\left\{\mathbf{x}\in \mathbb{R}^{\Dim}
       :  g_i(\mathbf{x})\ge 0\right\}.
   \end{equation}
  The $g_i$'s are called the \emph{generating functions}
   of ${\mathcal S}$.
  In particular, a semianalytic set is \emph{semialgebraic}
  if all of its generating functions are polynomials.
\end{definition}

Recall that a function is \emph{analytic}
 if and only if
 its Taylor series at $\mathbf{x}_0$
 converges to the function in some neighborhood
 for every $\mathbf{x}_0$ in its domain.
In the example of (\ref{eq:pathologicalIntersection}),
 ${\mathcal A}_s$ is semianalytic while 
 ${\mathcal A}_p$ is not,
 because the Taylor series of $g_2(x,y):=\sin\frac{1}{x}-y$
 at the origin does not converge.
Roughly speaking,
 the boundary curves of regular semianalytic sets
 are piecewise smooth.
% By restricting our attention to regular closed or open sets
%  ${\mathcal S}$ which are also semianalytic,
%  we can be sure that for each $\mathbf{x}\in{\mathcal S}$
%  and any sufficiently small $r>0$,
%  the intersection of ${\mathcal S}$
%  to the open ball at $x$ with radius $r$
%  can be described by a finite set
%  of ``well-behaved'' functions.


 \begin{figure}[H]
  \centering 
  {\includegraphics[width=0.6\textwidth]{png/yinsetexm}}
  \caption{An example of a bounded 3D Yin set. The Yin set
    consists of two components: one is a big torus with a
    ball and a small torus removed, the other is a big torus with
    a small torus removed.
  }
  \label{fig:yinsetexm}
 \end{figure}
\subsection{$\mathbb{Y}$:  
  the Yin space for fluid modeling}
\label{sec:YinSpace}

Regular closed semianalytic sets have been
 an essential mathematical tool
 for solid modeling
 since the dawning time of this field
 \cite{requicha78:_mathem_found_const_solid_geomet}.
However,
 the boundary representation
 of a regular closed semianalytic set
 is not unique;
 see \cite[Fig. 5]{zhang20:_boolean} for an illustration.
As another work closely related to this one,
 the analysis on a family of interface tracking methods
 \cite{zhang13:VOFadvection,zhang16:_mars}
 via the theory of donating regions
 \cite{zhang13:_donat_region,zhang15:_gener_donat_region}
 also requires that the regular sets be open.
Therefore,
 only regular open semianalytic sets are employed in this work.

\begin{definition}
  \label{def:YinSet}
  A \emph{Yin set}\footnote{
    Yin sets are named after the first author's mentor,
    Madam Ping Yin.
    As a coincidence,
     the most important dichotomy in Taoism
     consists of Yin and Yang,
     where Yang represents the active, the straight, the ascending,
     and so on, 
     while Yin represents the passive, the circular, the descending,
     and so on.
  From this viewpoint, straight lines and Jordan curves can be 
   considered as Yang 1-manifolds and Yin 1-manifolds, respectively.
  } $\mathcal{Y}\subseteq \mathbb{R}^D$
   is a regular open semianalytic set
   whose boundary is bounded.
  The class of all such Yin sets form
   the \emph{Yin space} $\mathbb{Y}$.
\end{definition}

Hereafter we focus on the case of $D = 3$.
Figure \ref{fig:yinsetexm} gives an example of a bounded 3D Yin set.
% By Definition \ref{def:semianalytic-sets},
%  semianalytic sets are closed under
%  set complementation, finite union, and finite intersection.
% % they are also closed under topological operations.
% Then by Theorem \ref{thm:regularOpenAlgebra},
%  regular open semianalytic sets
%  form a Boolean algebra
%  since they are the intersection of the universes
%  of two Boolean algebras.
% Furthermore,
%  Boolean operations on Yin sets
%  preserve the attribute of
%  a bounded boundary being bounded,
%  hence we have
 
%  \begin{theorem}
%    \label{thm:YinSetsFormABooleanAlgebra}
%     The algebra
%     $\mathbf{Y}:=({\mathbb Y},\ \cup^{\perp\perp},\ \cap,\ \, ^{\perp},\
%     \emptyset,\ \mathbb{R}^2)$
%     is a Boolean algebra.
%  \end{theorem}

% \subsection{Jordan curves and orientations}
% \label{sec:JordanCurves}

% A \emph{path} in $\mathbb{R}^2$ from $p$ to $q$
%  is a continuous map $f:[0,1]\rightarrow \mathbb{R}^2$
%  satisfying $f(0)=p$ and $f(1)=q$.
% A subset ${\mathcal P}$ of $\mathbb{R}^2$
%  is \emph{path-connected} if
%  every pair of points of ${\mathcal P}$
%  can be joined by a path in ${\mathcal P}$.
% Given ${\mathcal Q}\subset \mathbb{R}^2$,
%  define an equivalence relation on ${\mathcal Q}$
%  by setting $x\sim y$ if there is a path-connected subset of $Q$
%  that contains both $x$ and $y$.
% The equivalence classes are called
%  the \emph{path-connected component}s of ${\mathcal Q}$.

% A \emph{planar curve} % in $\mathbb{R}^{\Dim}$
%  is a continuous map
%  $\gamma: (0,1) \rightarrow \mathbb{R}^{2}$.
% %It is \emph{smooth} if the map is smooth.
% It is \emph{piecewise analytic} if the map is
%  the composite of a finite number of analytic functions.
% It is \emph{simple} if the map is injective;
%  otherwise it is \emph{self-intersecting}.
% Although strictly speaking a curve $\gamma$ is a map,
%  we also use $\gamma$ to refer to its image.
% Two distinct curves $\gamma_1$ and $\gamma_2$
%  \emph{intersect} at $q$ if there exist $s_1,s_2\in (0,1)$
%  such that \mbox{$\gamma_1(s_1)=\gamma_2(s_2)=q$}.
% Then $q$ is the \emph{intersection} of $\gamma_1$ and $\gamma_2$.
% For an open ball ${\mathcal N}_r(q)$ with sufficiently small radius $r$,
%  ${\mathcal N}_r(q)\setminus\gamma_1$ consists of
%  two disjoint connected regular open sets.
% If $\gamma_2\setminus q$ is 
%  entirely contained in one of these two sets,
%  $q$ is an \emph{improper intersection};
%  otherwise it is a \emph{proper intersection}.
% % illustrated in Figure \ref{fig:localTopology} (b).
% %
% Two curves are \emph{disjoint} if
%  they have neither proper intersections nor improper ones.
% %
% Suppose upon its extension to a path,
%  a simple curve $\gamma$ further satisfies
%  $\gamma(0)=\gamma(1)$,
%  then $\gamma$ is
%  a \emph{simple closed curve} or \emph{Jordan curve}. % (SCC)

% \begin{theorem} [Jordan Curve Theorem \cite{jordan87:_cours_daanl_polyt}]
%  \label{thm:jordan}
%  The complement of a Jordan curve $\gamma$
%  in the plane $\mathbb{R}^2$
%  consists of two components,
%  each of which has $\gamma$ as its boundary.
%  One component is bounded and the other is unbounded;
%  both of them are open and path-connected.
% \end{theorem}

% The above theorem states that a Jordan curve divides the plane
%  into three parts: itself, its \emph{interior},
%  and \emph{exterior}.

% \begin{definition}
% \label{def:interior}
% The \emph{interior} of an oriented Jordan curve $\gamma$,
%  denoted by $\Int(\gamma)$,
%  is the component of the complement of $\gamma$
%  that always lies to the left
%  when an observer traverses the curve
%  in the increasing direction of the parameterization $s$.
% \end{definition}

% A Jordan curve is said to be \emph{positively oriented}
%  if its interior is the bounded component of its complement;
%  otherwise it is \emph{negatively oriented}.
% The orientation of a Jordan curve
%  can be flipped
%  by reversing the increasing direction of the parameterization.
% The following notion will be used throughout this work.

% \begin{definition}
%   \label{def:almostDisjoint}
%   Two Jordan curves are 
%    \emph{almost disjoint}
%    if they have no proper intersections
%    and at most a finite number of improper intersections.
% \end{definition}


\subsection{Compact 2-manifolds}
\label{sec:compact-2-manifolds}

An \emph{$m$-manifold} is a Hausdorff space $X$
with a countable basis such that each point $x\in X$
has a neighborhood that is homeomorphic
with an open subset of $\mathbb{R}^m$.
A 1-manifold is often called a curve
and a 2-manifold is called a \emph{surface}.

Let $\mathcal{M}$ be a compact smooth surface.  
At each point $p \in \mathcal{M}$, the tangent space $T_p \mathcal{M}$ is a
2D real vector space.  
If $(v_1,v_2)$ and $(v_1',v_2')$
are two ordered bases of $T_p \mathcal{M}$ such that
$\det([v_1',v_2']) > 0$
relative to $(v_1,v_2)$, they determine the same orientation class.
$\mathcal{M}$ is said to be \emph{orientable} if
such a continuous choice exists.
The following well known theorem is a classification
of orientable compact surfaces.

\begin{theorem}[\cite{massey77:_alg_topo_an_intro}]
  \label{thm:manifoldclassification}
  Every orientable compact surface is homeomorphic 
  either to a sphere or to a connected sum of tori.
\end{theorem}

 
The classical Jordan Curve Theorem \cite{jordan87:_cours_daanl_polyt}
establishes that every simple
closed curve in $\mathbb{R}^{2}$ divides the plane into
a bounded and an unbounded region.
As an key extension, the Jordan-Brouwer Separation Theorem
\cite[Theorem 6.35]{rotman88:_intro_to_alge_topo}
generalizes this to higher dimensions
by proving that any $(n-1)$-sphere embedded in $\mathbb{R}^{n}$
induces the same separation.
Subsequent researches
\cite{lima88:_jordan_brouwer_separation_theorem_for_hype,
  _schmaltz09:_jordan_brouwer_separation_theorem} extend this result  
to orientable compact surfaces.

For an orientable compact surface $\mathcal{M}$ and a local
ordered bases $(v_1,v_2)$ of $T_p \mathcal{M}$,
the induced normal vector $n$ is the one such that
$(v_1,v_2,n)$ forms a right-handed frame in $\mathbb{R}^3$.
Then $\mathcal{M}$ is \emph{positively oriented} if $n$
points from the bounded complement of $\mathcal{M}$
to the unbounded complement; otherwise it is \emph{negatively oriented}.
The \emph{interior of a positively oriented compact surface}
 is its bounded complement
 and 
 the \emph{interior of a negatively oriented compact surface}
 is its unbounded complement.
 The other complement is defined as the \emph{exterior} of the surface.

% An orientable compact surface has
%  the \emph{positive orientation}
%  if the outward norm vector of the surface
%  points from the bounded complement of the surface
%  to the unbounded complement; 
%  otherwise it has the negative orientation.
% The \emph{interior of a positively oriented compact surface}
%  is its bounded complement
%  and 
%  the \emph{interior of a negatively oriented compact surface}
%  is its unbounded complement.
 
% A \emph{surface patch} is (the image of) a continuous function
% $(0,1)^2 \rightarrow \mathbb{R}^3$.
% Two surface patches $S_1$ and $S_2$
% \emph{do not intersect}
% if $S_1\cap S_2 = \emptyset$; 
% otherwise a point $p\in S_1\cap S_2$
% is called a \emph{proper intersection} of  $S_1$ and $S_2$
% if for all sufficiently small neighborhood ${\cal N}(p)\subset \mathbb{R}^3$
% both of the two connected components of ${\cal N}(p)\backslash S_2$
% contain part of $S_1$
% and both components of ${\cal N}(p)\backslash S_1$ contain part of $S_2$. 
% Two surface patches $S_1$ and $S_2$
%  are said to \emph{intersect improperly}
%  if $S_1\cap S_2 \ne \emptyset$
%  but none of the intersection points is a proper intersection.
% The above concepts generalize in a straightforward way to compact surfaces. 
 



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../YinSets3D"
%%% End:

